An Autoregressive Model for Time Series of Random Objects

Random variables in metric spaces indexed by time and observed at equally spaced time points are receiving increased attention due to their broad applicability. The absence of inherent structure in metric spaces has resulted in a literature that is predominantly non-parametric and model-free. To address this gap in models for time series of random objects, we introduce an adaptation of the classical linear autoregressive model tailored for data lying in a Hadamard space. The parameters of interest in this model are the Fr\'echet mean and a concentration parameter, both of which we prove can be consistently estimated from data. Additionally, we propose a test statistic for the hypothesis of absence of serial correlation and establish its asymptotic normality. Finally, we use a permutation-based procedure to obtain critical values for the test statistic under the null hypothesis. Theoretical results of our method, including the convergence of the estimators as well as the size and power of the test, are illustrated through simulations, and the utility of the model is demonstrated by an analysis of a time series of consumer inflation expectations.

==> sec_conclusion.tex <==
\section{Conclusion}

==> subsec_bootstrap.tex <==
\subsection{Bootstrapping moments of $D_T$ under $H_0$}\label{subsec_bootstrap}

\begin{algorithm}
    \caption{Estimation of the mean and variance of $D_T$ under $H_0$}\label{alg-bootstrap}
    \begin{algorithmic}
        \Require $X_1, \ldots, X_T$
        \Require $B \geq 0$
        
        \For{$b = 1, \ldots, B$}
        \State $\pi^{(b)} = $ random permutation of $\eset{1, \ldots, T}$
        \State $D^{(b)}_T = \frac{1}{T-1}\sum_{t=1}^{T-1} d(X_{\pi^{(b)}_t}, X_{\pi^{(b)}_{t+1}})^2.$
        \EndFor

        \State $\hat{\mathbb{E}}[D_T] = \frac{1}{B}\sum D_T^{(b)}$
        \State $\hat{\sigma}_0^2 = \frac{1}{B}\sum (D_T^{(b)} - \hat{\mathbb{E}}[D_T])^2$

        \State \textbf{return} $\hat{\mathbb{E}}[D_T], \hat{\sigma}_0^2$
    \end{algorithmic}
\end{algorithm}

As mentioned previously, the test above requires estimating the mean and variance of $D_T$ under $H_0$. To that end, we use a bootstrapping procedure combined with permutations of the sample. The procedure is detailed in the display of Algorithm \ref{alg-bootstrap}.

We currently do not have results available showing that the bootstrap is consistent, but we believe that standard bootstrap theory should yield the desired asymptotic result for the test based on critical values obtained using Algorithm \ref{alg-bootstrap}. For this reason, we can only state the following as a conjecture.

\begin{conjecture}
    Under $H_0$, for $\alpha \in (0,1)$,
    \begin{equation*}
        \limsup_{T \rightarrow \infty} \P{\sqrt{T}\abs{D_T - \hat{\mathbb{E}}[D_T]} \geq \hat\sigma_0 \Phi^{-1}(1 - \alpha / 2)} = \alpha.
    \end{equation*}
\end{conjecture}

{\color{red}
\begin{enumerate}
    \item Need to replace the hat critical values with star critical values.
    \item Show that $D_T^* - D_T \rightarrow_{d^*} N(0, 1)$
    \item Conclude that $\limsup_{T \rightarrow \infty} \P{\sqrt{T}\abs{D_T - \hat{\mathbb{E}}[D_T]} \geq \hat\sigma_0 \Phi^{-1}(1 - \alpha / 2)} = \alpha.$
\end{enumerate}
}

==> subsec_psd.tex <==
\subsection{PSD Matrices}

Let $\mathbb{S}^+_p$ denote the space of $p \times p$ symmetric positive definite matrices.
%
\begin{align*}
    d(A, B)
    = \norm{ \log(B^{-1/2}AB^{-1/2})}_F
    = \norm{ \log(B^{-1}A)}_F
    = \sum_{k=1}^p \log\left(\lambda_k(B^{-1}A)^2\right)
\end{align*}
%
Define the following class of isomorphisms: for $X \in GL_p$, let $\Gamma_X : 
\mathbb{S}^+_p \rightarrow \mathbb{S}^+_p$ be $\Gamma_X A = XAX^\top$. Then indeed $d(\Gamma_X A, \Gamma_X B) = d(A, B)$.

Let $\Sigma$ be a random matrix in $\mathbb{S}^+_p$ with mean $\mathbbm{1}_p$, then, consider the following noise structure
\begin{equation*}
    \varepsilon_\Sigma(A) = \Gamma_{A^{1/2}} \Sigma = A^{1/2} \Sigma A^{1/2}.
\end{equation*}
We have that
\begin{align*}
    &\expec{d(\varepsilon_\Sigma A, \omega)^2} = \expec{d(\Gamma_{A^{1/2}} \Sigma, \omega)^2}\\
    &= \expec{d(\Gamma_{A^{1/2}} \Sigma, \Gamma_{A^{1/2}}\Gamma_{A^{-1/2}}\omega)^2} 
    = \expec{d(\Sigma, \Gamma_{A^{-1/2}}\omega)^2} 
\end{align*}
and so
\begin{equation*}
    \expec{\varepsilon_\Sigma A}
    = \argmin_\omega \expec{d(\Sigma, \Gamma_{A^{-1/2}}\omega)^2} 
    = \Gamma_{A^{1/2}} \expec{\Sigma}
    = A^{1/2} \mathbbm{1}_p A^{1/2}
    = A.
\end{equation*}



\begin{equation*}
    \Gamma_{\mu^{\frac{1}{2}}}\expec{ \gamma_{\mathbbm{1}}^{\Gamma_{\mu^{-\frac{1}{2}}}X}\theta }
    = \Gamma_{\mu^{\frac{1}{2   }}}\expec{ (\mu^{-\frac{1}{2}}X\mu^{-\frac{1}{2}})^\theta }
    = \expec{\mu^{\frac{1}{2}}(\mu^{-\frac{1}{2}}X\mu^{-\frac{1}{2}})^\theta\mu^{\frac{1}{2}}}
    = \expec{\gamma_{\mu}^X \theta}
\end{equation*}
And since $\expec{\Gamma_{\mu^{-1/2}}X} = \mathbbm{1}$, wlog we can assume $\expec{X} = \mathbbm{1}$.

So now one has to show that for $\expec{X} = \mathbbm{1}$, we have $\expec{X^t} = \mathbbm{1}$.
%
\begin{align*}
    &X^t = \exp\left(t \log X\right) = W \Lambda^t W^\top\\
    &d(X^t, \omega)^2
\end{align*}

==> subsec_useful_results.tex <==
\subsection{Useful results}


